Discourse Understanding and Factual Consistency in Abstractive Summarization

We introduce a general framework for abstractive summarization with factual consistency and distinct modeling of the narrative flow in an output summary. Our work addresses current limitations of models for abstractive summarization that often hallucinate information or generate summaries with coherence issues. To generate abstractive summaries with factual consistency and narrative flow, we propose Cooperative Generator -- Discriminator Networks (Co-opNet), a novel transformer-based framework where a generator works with a discriminator architecture to compose coherent long-form summaries. We explore four different discriminator objectives which each capture a different aspect of coherence, including whether salient spans of generated abstracts are hallucinated or appear in the input context, and the likelihood of sentence adjacency in generated abstracts. We measure the ability of Co-opNet to learn these objectives with arXiv scientific papers, using the abstracts as a proxy for gold long-form scientific article summaries. Empirical results from automatic and human evaluations demonstrate that Co-opNet learns to summarize with considerably improved global coherence compared to competitive baselines.

==> 4-setup.tex <==
\section{Experimental Setup}
\jan{Don't need a seperate section on this.}
%In this section we outline comparison baselines and describe experimental setups for our generator and discriminator models.

\subsection{Baselines}

We compare against extractive approaches using Lede-3, SumBasic \cite{Vanderwende2007BeyondST}, LSA \cite{Steinberger2004UsingLS} and LexRank \cite{Erkan2004LexRankGC} baselines. We also compare three state-of-the-art abstractive approaches: a 2-layer bi-LSTM sequence-to-sequence model with attention, and a pointer-generator model \cite{see2017get} and a discourse-aware LSTM model \cite{cohan2018discourse}. 
Additional implementation details are given in the Appendix \antoine{which Appendix?}. 

\subsection{Our Model}

\noindent \textbf{Implementation} All our models are implemented in Pytorch. Our generator and discriminator code is adapted from the OpenAI Huggingface\footnote{\url{ https://github.com/huggingface/transformers}} implementation of the Bert and GPT-2 language model\footnote{Our code/data is available here: \url{https://github.com/coopnet-model}.} %\footnote{Due to the memory constraints of our 12GB Titan-X GPU, we were unable to run experiments with the GPT-2 Medium model using the full 1024 context size. Since the full context is necessary for capturing details related to results sections and main contributions that tend to appear at the end of introductions, we forgo using the GPT-2 Medium model.}  
and uses the pre-trained weights of \citet{Radford2019LanguageMA}. 

\noindent \textbf{Training} We use a learning rate of 2e-5 for finetuning. We use a batch size of 1 with gradient accumulation to simulate a batch size of 16 for finetuning the generator, and a batch size of 2 for finetuning the discriminator. 

\noindent \textbf{Generation Hyperparameters} During inference time, we use top-$k$ sampling with $k$=4 \cite{Fan2018HierarchicalNS} %or nucleus sampling with p =.9 \cite{holtzman2019curious} 
to generate 10 candidate summaries for each model. In the re-ranking objective (Equation~\ref{eq:final_gen_score}), we weigh the generation and discriminator models equally for all experiments by setting $\lambda_{gen} = \lambda_{disc} = .5$. %and select the candidate out of the 10 that achieves the highest joint score in Equation~\ref{eq:final_gen_score} to be the final summary. 
%We also convert sentences generated from the GPT-2 base summarization model by mapping the GPT-2 tokenization to BERT WordPiece tokenization with the SciBERT vocabulary. 
 %A clearly non-coherent candidate summary is effectively removed from consideration by the discriminator by setting the adjacency score to $-\infty$. 

% \indent To optimize decoding time, we compute all pairwise sentence adjacency comparisons for a given candidate summary in parallel. Since sentence pairs are of varying lengths, we pad the sentence pairs to a fixed length based on the longest sentence pair. 



==> experiments/abstractiveness.tex <==



==> experiments/analysis.tex <==
\subsection{Impact of Discriminator}

\begin{table*}[t]
\centering
    \resizebox{\textwidth}{!}{\begin{tabular}{l|c|ccc|ccr}
    \toprule
    Model & Task & BERT-P & BERT-R & BERT-F1 & SCIBERT-P & SCIBERT-R & SCIBERT-F1 \\
    \midrule
    PGen + Coverage \cite{see2017get} &  First-50 & 57.17 & 55.79 & 56.30 & 60.23 & 59.31 & 59.70 \\
    Base (topk,k=4) & First-50 & 59.16 & 54.72 & 56.72 & 62.97 & 59.42 & 61.05 \\
    \model~(topk, k=4) & First-50  & 57.76 & 55.95 & 56.74 & 61.57 & 60.28 & 60.86 \\
    \midrule
    PGen + Coverage \cite{see2017get} &  Last-50 & 53.55 & 52.45 & 52.90 & 57.29 & 56.52 & 56.84 \\
    Base (topk,k=4) & Last-50 & 55.58 & 51.76 & 53.48 & 59.96 & 56.73 & 58.23 \\
    \model~(topk, k=4) & Last-50  & 53.95 & 52.29 & 53.04 & 58.13 & 56.89 & 57.45 \\
    \midrule
    PGen + Coverage \cite{see2017get} &  Overall & 60.44 & 55.88 & 57.86 & 61.15 & 57.53 & 59.13 \\
    Base (topk,k=4) & Overall & \textbf{63.17} & 52.25 & 57.00 & \textbf{65.27} & 56.08 & \textbf{60.20}\\
    \model~(topk, k=4) & Overall  & 60.66 & \textbf{56.23} & \textbf{58.21} & 62.03 & \textbf{58.51} & 60.11 \\
    \bottomrule
    \end{tabular}
    }
\caption{BERTScore results for AAN dataset}
\label{table:fullbertscore}
\end{table*}

\begin{table*}[t]
\centering
    \resizebox{\textwidth}{!}{\begin{tabular}{l|c|ccc|ccr}
    \toprule
    Model & Dataset & BERT-P & BERT-R & BERT-F1 & SCIBERT-P & SCIBERT-R & SCIBERT-F1 \\
    \midrule
    PGen + Coverage \cite{see2017get} &  CS~\dataset &  & &  &  & &  \\
    Base (topk,k=4) & CS~\dataset  & 61.88 & 52.47 &  56.66 &  62.52 &  54.98 & 58.42\\
    \model~(topk, k=4) & CS~\dataset   & 60.21 & 54.49 & 57.08 & 59.89 & 55.76 & 57.66 \\
    \midrule
    
    PGen + Coverage \cite{see2017get} &  Bio~\dataset & &  &  &  &  & \\
    Base (topk,k=4) & Bio~\dataset & 59.16 & 50.57 & 54.42 & 59.25 & 52.93 & 55.84 \\
    \model~(topk, k=4) & Bio~\dataset  & 57.54 & 51.93 & 54.49 & 56.60 & 53.23 & 54.80 \\
    \midrule
    
    PGen + Coverage \cite{see2017get} &  AAN & 60.44 & 55.88 & 57.86 & 61.15 & 57.53 & 59.13 \\
    Base (topk,k=4) & AAN & 63.17 & 52.25 & 57.00 & 65.27 & 56.08 & 60.20\\
    \model~(topk, k=4) & AAN & 60.66 & 56.23 & 58.21 & 62.03 & 58.51 & 60.11 \\
    \bottomrule
    \end{tabular}
    }
\caption{Overall BERTScore results for all \dataset~subsets and AAN dataset}
\label{table:allbertscore}
\end{table*}

\begin{table}[H]
\begin{center}
\resizebox{\columnwidth}{!}{%
    \begin{tabular}{ l | r | r }
    \toprule
    Model  & Avg \# Words  & \% New Decision \\ \toprule
    % Base (nucleus,p=.9)  &  71.04 & \NA  \\ 
    % \model~(nucleus, p=.9) & 104.91  & 95.9 \\ 
    Base (topk,k=4)  &  49.11 & \NA  \\ 
    \model~(topk, k=4) & 86.40  & 97.6 \\
    \end{tabular}
    
}

\caption{Analysis of how often the discriminator changes the sequence selected as the top candidate.}
\label{table:comp}
\end{center}
    \end{table}
    
\begin{table}[H]
\begin{center}
\resizebox{\columnwidth}{!}{
    \begin{tabular}{ l | r | r | r |}
    \toprule
    Model  & \% Overlap-1 & \% Overlap-2  & \% Discourse (n=1)     \\ \toprule
    % Base (nucleus,p=.9)  &  71.04 & \NA  \\ 
    % \model~(nucleus, p=.9) & 104.91  & 95.9 \\ 
    Base (topk,k=4)  & 8.42  & 0.03 & 6.02  \\ 
    \model~(topk, k=4) & 8.64  & 0.08 & 6.20 \\
    \end{tabular}
    }
\caption{Analysis of how well \model~captures discourse in AAN generations compared to the Base model.}
\label{table:disc}
\end{center}
    \end{table}
    
\paragraph{Capturing Discourse} We also evaluate the ability of \model~to capture discourse terms. Discourse lexical terms are defined using the English discourse connectives lexicon from the work of \cite{Das2018ConstructingAL}.\footnote{\url{https://github.com/discourse-lab/en\_dimlex}} We measure how well discourse terms are captured by computing the average percentage of overlapping n-grams between the generated summary and the gold summary that are related to discourse for n = 1 (\% Overlap-1) and n = 2  (\% Overlap-2). Additionally, we compute the the average percentage of unigrams (\% Discourse) in the generated summary that are discourse terms. Results in Table \ref{table:disc} show that \model~generations capture slightly more discourse terms from the gold summary and overall contain a higher percentage of discourse terms than generations from the Base model. 



==> experiments/bert_score.tex <==
%\subsection{Alternatives to ROUGE}
%\label{ssec:beyond}

%Despite our generally superior results on the ROUGE metric, past work \cite{Schluter2017TheLO,Hoang2019EfficientAO,Sun2019HowTC} has explored the limitations of ROUGE for evaluating summarization tasks, including the issue that ROUGE measures $n$-gram overlap without distinguishing between salient $n$-grams and non-contentful tokens. This failure means that models with a higher probability of generating generic, frequent terms such as ``the'' and ``how'' can potentially outperform models that better capture conceptual information, but may paraphrase rather than extract common terms. 

%To overcome these limitations, we explore using contextualized evaluation to measure how well models learn to extract conceptual meaning from scientific paper introductions and generate high-quality abstracts. The BERTScore metric \cite{Zhang2019BERTScoreET}, which has been shown to be well correlated with human judgments on other NLP tasks, is one such metric that measures similarity between contextual embeddings of the generated summary and reference summary. For a generated %abstract $\hat{S} = \{\hat{x}_1,...,\hat{x}_n\}$ of length $\hat{n}$ 
%and gold abstract, we first convert the sequences of tokens into sequences of contextual vector representations using either the uncased version of BERT-base or the SciBERT variant. Following \cite{Zhang2019BERTScoreET}, we then compute precision, recall and F1 scores from these contextual representations.

%%$S^* = \{x^*_1, ..., x^*_n\}$ of length $n^*$

%% :
%% \[BERT-P = \frac{\sum_{\hat{x}_i \in \hat{x}} idf(\hat{x}_i)max_{x_j \in x} \textbf{x}_i^T \hat{\textbf{x}}_j}{\sum_{\hat{x}_i \in \hat{x}} idf(\hat{x}_i)}\]
%% \[BERT-R = \frac{\sum_{x_i \in x} idf(x_i)max_{\hat{x_j} \in \hat{x}} \textbf{x}_i^T \hat{\textbf{x}}_j}{\sum_{x_i \in x} idf(x_i)}\]
%% \[BERT-F1 = 2 \cdot \frac{BERT-P \cdot BERT-R}{BERT-P + BERT-R}\], 
%% where idf is defined as the inverse document frequency score. 

%%We consider three separate evaluation tasks, based on the observation that abstracts generated from the PGen + Coverage model \cite{see2017get} lack completeness in terms of including details about the approach and results when compared to the transformer models (see Figure \ref{fig:errors} in section 8 for more details). In the First-50 and Last-50 tasks, we only consider the first 50 and last 50 tokens of abstracts, respectively. In the overall task, we consider the entire abstract.

%\paragraph{Results} Our results on the BERTScore evaluation reinforce our observations from the human and ROUGE score evaluations. \model~generally outperforms the PGen + Coverage baseline across all metrics, regardless of the evaluation model used (BERT, SciBERT). Results are more mixed when comparing \model~to the base model with no discriminator. Overall, \model~is less precise than the Base model at capturing contextual meaning, potentially due to the fact that the \model~tends to produce longer summaries (86.4 tokens vs.~49.11 tokens for Base) and \model~generations contain slightly more discourse-aware transitional terms composed of stopwords (See Table \ref{table:disc} in the Appendix).  %inclusion of more sequential terms (for example, ``first" or ``lastly") and transitional keyphrases (e.g. ``using the given approach") that do not provide more conceptual meaning but positively impact narrative flow\footnote{Note that candidate summaries selected by the Base + Disc model are considerably longer on average than the Base model generations. See Table \ref{table:comp} in the Appendix for details.}. 
%This observation is supported by the fact that \model~achieves the best results in terms of recall, beating the Base model by 3.98 points on BERT-R and 2.43 points on SciBERT-R.










==> experiments/concept_rouge.tex <==
Due to the limitations of ROUGE in showing how generated summaries capture contentful information, we introduce a variant of ROUGE focused on conceptual overlap between generated summaries and gold summaries by only considering words contained in n-grams that are not stopwords. 

\begin{table}
\centering
\resizebox{\columnwidth}{!}{%
    \begin{tabular}{ l | r r r }
    \toprule
    Model & R-1 Precision & R-1 Recall & R-1 F1 \\ 
    \midrule
    Base (nucleus, p = .9) & 31.56 & 20.47 & 23.60 \\
    \model~(nucleus, p = .9)  &  24.78 & 24.31  & 23.78 \\ \midrule Model & R-L Precision & R-L Recall & R-L F1 \\ \midrule
    Base (nucleus, p = .9) &  29.13 & 18.84 & 21.74 \\
    \model~(nucleus, p = .9)  &  22.79 & 22.30  & 21.85 \\
    \bottomrule
    \end{tabular}
    }
\caption{Comparison of ROUGE for AAN abstracts generated from transformer models with stopwords removed }
\end{table}


Our results (see Table 7) show that the discriminator model slightly outperforms the base transformer model. To build on this approach, we look at more contextual measures of generation quality. 

==> experiments/mturk_setup.tex <==
%\newpage
\begin{figure*}
\begin{subfloat}
    \centering 
    \includegraphics[width=1\textwidth]{figures/1.png}
    \label{fig:1}
\end{subfloat}
\begin{subfloat}
    \centering
    \includegraphics[width=1\textwidth]{figures/2.png}
    \label{fig:2}
\end{subfloat}
\begin{subfloat}
    \centering
    \includegraphics[width=1\textwidth]{figures/3.png}
    \label{fig:3}
\caption{Amazon MTurk setup for expert eval}
\end{subfloat}
\end{figure*}

==> experiments/wiki_results.tex <==
\begin{table}[ht!]
\begin{center}
\resizebox{\columnwidth}{!}{%
    \begin{tabular}{ l | r | r | r }
    \hline
    Model & Rouge-1 & Rouge-2 & Rouge-L \\ \hline
    Lede-3 & 0.2600 & 0.0724 &  0.2425 \\
    LSTM &  0.2204 & 0.0627 & 0.2087  \\ 
    LSTM + PG & 0.2853 & 0.0923 & 0.2654    \\
    Transformer (topk) & 0.2813 & 0.0677 & 0.2697  \\
    Transformer + Discriminator (topk)  &  0.2875 & 0.0607  & 0.2733 \\
    Transformer (beam) & 0.3316 & 0.1271 & 0.3199  \\
    \end{tabular}
}
\caption{WikiHow Article to Summary Task}
\end{center}
    \end{table}
